Routing and Wavelength Assignment with Protection: A Quadratic Unconstrained Binary Optimization Approach

The routing and wavelength assignment with protection is an important problem in telecommunications. Given an optical network and incoming connection requests, a commonly studied variant of the problem aims to grant maximum number of requests by assigning lightpaths at minimum network resource usage level, while ensuring the provided services remain functional in case of a single-link failure through dedicated path protection. We consider a practically relevant version where alternative lightpaths for requests are assumed to be given as a precomputed set, and show that it is NP-hard. We formulate the problem as an integer programming (IP) model, and also use it as a foundation to develop a novel quadratic unconstrained binary optimization (QUBO) model, which can be both directly solved by a state-of-the-art solver like GUROBI. We present necessary and sufficient conditions on objective function parameters to prioritize request granting objective over wavelength-link usage for both models, and a sufficient condition to ensure the exactness of the QUBO model. Moreover, we implement a problem-specific branch-and-cut algorithm for the IP model, and employ a new quantum-inspired technology, Digital Annealer (DA), for the QUBO model. We conduct computational experiments on a large suite of instances that are hard to optimally solve in order to assess the efficiency and efficacy of all of these approaches as well as a problem-specific heuristic. The results show that the emerging technology DA outperforms the considered established techniques coupled with GUROBI, in finding mostly significantly better or as good solutions in only two minutes compared to two hours of run time, whereas the problem-specific heuristic fails to be competitive.

==> IP_subfiles/lemma_beta_models_equiv.tex <==
\begin{corollary}
\label{lem:beta_models_equiv} %[?????]
The prioritization condition given in \eqref{eq:prioritization_optmodel0} can be achieved by setting $\alpha, \beta > 0$ such that 
$\frac{\beta}{\alpha}  >  \LBprioOne $

\end{corollary}



==> IP_subfiles/thm_NPhard_fig1.tex <==
\begin{figure}[!h]
\centering
\tikzset{main_node/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt},}
\tikzset{node1/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = red},}
\tikzset{node2/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = yellow},}
\tikzset{node3/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = blue!60!white},}
\tikzstyle{edge} = [draw,line width=1pt,-]
\tikzstyle{highlighted edge} = [draw,line width=6pt,-,green!70!black, opacity=0.3]
\scalebox{0.65}{
\begin{tikzpicture}

    \node[node1,minimum size=0.95cm] (u1) {\large $\mssnode_1$};
    \node[node2,minimum size=0.95cm] (u2) [below left = 0.5 cm and 0.5 cm of u1] {\large $\mssnode_2$};
    \node[node3,minimum size=0.95cm] (u3) [below right = 0.5 cm and 0.5 cm of u1]  {\large $\mssnode_3$};
    
    \path[edge]
         (u1) to (u2)
         (u1) to (u3);
    
    \begin{scope}[xshift=9cm, yshift=1cm]
        \node[node1] (s_1) {$s^1$};
        \node[main_node] (w_11) [above right = 0.25 cm and 1.25 cm of s_1] {$\wnode^1_1$};
        \node[main_node] (p_11) [below right = 0.25 cm and 1.25 cm of s_1]  {$\pnode^1_1$};
        \node[node1] (t_1) [below right = 0.25 cm and 1.25 cm of w_11]  {$t^1$};
        
        \path[edge]
             (s_1) edge[bend left=20]  (w_11)
             (w_11) edge[bend left=20] (t_1)
             (s_1) edge[bend right=20]  (p_11)
             (p_11) edge[bend right=20] (t_1);
    \end{scope}
    
    \begin{scope}[xshift=6cm, yshift=-2cm]
        \node[node2] (s_2) {$s^2$};
        \node[main_node] (w_21) [above right = 0.25 cm and 1.25 cm of s_2] {$\wnode^2_1$};
        \node[main_node] (p_21) [below right = 0.25 cm and 1.25 cm of s_2]  {$\pnode^2_1$};
        \node[node2] (t_2) [below right = 0.25 cm and 1.25 cm of w_21]  {$t^2$};
        
        \path[edge]
             (s_2) edge[bend left=20]  (w_21)
             (w_21) edge[bend left=20] (t_2)
             (s_2) edge[bend right=20]  (p_21)
             (p_21) edge[bend right=20] (t_2);
    \end{scope}
    
    \begin{scope}[xshift=12cm, yshift=-2cm]
        \node[node3] (s_3) {$s^3$};
        \node[main_node] (w_31) [above right = 0.25 cm and 1.25 cm of s_3] {$\wnode^3_1$};
        \node[main_node] (p_31) [below right = 0.25 cm and 1.25 cm of s_3]  {$\pnode^3_1$};
        \node[node3] (t_3) [below right = 0.25 cm and 1.25 cm of w_31]  {$t^3$};
        
        \path[edge]
             (s_3) edge[bend left=20]  (w_31)
             (w_31) edge[bend left=20] (t_3)
             (s_3) edge[bend right=20]  (p_31)
             (p_31) edge[bend right=20] (t_3);
    \end{scope}
       
    \node (info_node1) [below = 3.5 cm of u1] {(i) };
    \node (info_node2) [below = 3.75 cm of p_11] {(ii)};

\end{tikzpicture}
}
\caption{(i) An {\mss} instance $\exMSSinst$, (ii) the initial incomplete form of the corresponding {\PRWAreq} network $\exPRWAnetwork$ }
\label{fig:nphard_mss_to_init_paths}
\end{figure}	

==> IP_subfiles/thm_NPhard_fig2.tex <==
\begin{figure}[!h]
    \centering
     \tikzset{main_node/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt},}
    \tikzset{node1/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = red},}
    \tikzset{node2/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = yellow},}
    \tikzset{node3/.style={circle,draw,line width=0.75pt,minimum size=0.75cm,inner sep=0pt,fill = blue!60!white},}
    \tikzstyle{edge} = [draw,line width=1pt,-]
    \tikzstyle{highlighted edge} = [draw,line width=6pt,-,green!70!black, opacity=0.3]
    
    \scalebox{0.59}{
    \begin{tikzpicture}
    
        \node[node1] (s_1) {$s^1$};
        \node[main_node] (w_11) [above right = 0.25 cm and 1.25 cm of s_1] {$\wnode^1_1$};
        \node[main_node] (p_11) [below right = 0.25 cm and 1.25 cm of s_1]  {$\pnode^1_1$};
        \node[node1] (t_1) [below right = 0.25 cm and 1.25 cm of w_11]  {$t^1$};
        
        \path[edge]
             (s_1) edge[bend left=20]  (w_11)
             (w_11) edge[bend left=20] (t_1)
             (s_1) edge[bend right=20]  (p_11)
             (p_11) edge[bend right=20] (t_1);
             
        \begin{scope}[yshift=-3.25cm]
            \node[node2] (s_2) {$s^c$};
            \node[main_node] (w_21) [above right = 0.25 cm and 1.25 cm of s_2] { $\wnode^2_1$};
            \node[main_node] (p_21) [below right = 0.25 cm and 1.25 cm of s_2]  {$\pnode^2_1$};
            \node[node2] (t_2) [below right = 0.25 cm and 1.25 cm of w_21]  {$t^2$};
            
            \node (info1) [below = 0.5 cm of p_21]  {(i)};

            \path[edge]
                 (s_2) edge[bend left=20]  (w_21)
                 (w_21) edge[bend left=20] (t_2)
                 (s_2) edge[bend right=20]  (p_21)
                 (p_21) edge[bend right=20] (t_2);
        \end{scope}
        
        \begin{scope}[xshift=6.5cm]
            \node[node1] (s_1) {$s^1$};
            \node[main_node] (w_11) [above right = 0.25 cm and 1.25 cm of s_1] {$\wnode^1_1$};
            \node[main_node] (w_12) [right = 1.15 cm of w_11] {$\wnode^1_2$};
            \node[main_node] (p_11) [below right = 0.25 cm and 1.25 cm of s_1]  {$\pnode^1_1$};
            \node[node1] (t_1) [below right = 0.25 cm and 1.25 cm of w_12]  {$t^1$};
            
            \node (trans_node_1) [below left = 1 cm and 1.25 cm of s_1] {};
            \node (trans_node_2) [below left = 1 cm and 0.5 cm of s_1] {};
            \draw[ultra thick,->] (trans_node_1) to (trans_node_2);
            
            \path[edge]
                 (s_1) edge[bend left=20]  (w_11)
                 (w_11) edge[bend left=5] (w_12)
                 (w_12) edge[bend left=20] (t_1)
                 (s_1) edge[bend right=20]  (p_11)
                 (p_11) edge[bend right=20] (t_1);
        \end{scope}
        
        \begin{scope}[xshift=6.5cm, yshift=-3.25cm]
            \node[node2] (s_2) {$s^2$};
            \node[main_node] (w_21) [above right = 0.25 cm and 1.25 cm of s_2] { $\wnode^2_1$};
            \node[main_node] (w_22) [right = 1.15 cm of w_21] { $\wnode^2_2$};
            \node[main_node] (p_21) [below right = 0.25 cm and 1.25 cm of s_2]  {$\pnode^2_1$};
            \node[node2] (t_2) [below right = 0.25 cm and 1.25 cm of w_22]  {$t^2$};

            \node (info1) [below right = 0.5 cm and 0.25 cm of p_21]  {(ii)};

            \path[edge]
                (s_2) edge[bend left=20]  (w_21)
                (w_21) edge[out=30,in=-80] (w_11)
                (w_22) edge[out=150,in=-80] (w_12)
                %(w_12) edge[out=-80,in=150] (w_22)
                (w_22) edge[bend left=20] (t_2)                    
                (s_2) edge[bend right=20]  (p_21)
                (p_21) edge[bend right=20] (t_2);
                
            \path[highlighted edge]
                (s_2)  to[bend left=20]  (w_21)
                (w_11) to[bend left=5] (w_12)
                (w_21) to[out=30,in=-80] (w_11)
                (w_12) to[out=-80,in=150] (w_22)
                (w_22) to[bend left=20] (t_2); 
            \path[edge]
                (w_11) edge[line width = 2.5pt, bend left=5] (w_12);
        \end{scope}
        
        \begin{scope}[xshift=14.5cm]
            \node[node1] (s_1) {$s^1$};
            \node[main_node] (w_11) [above right = 0.25 cm and 1.25 cm of s_1] {$\wnode^1_1$};
            \node[main_node] (w_12) [right = 1.15 cm of w_11] {$\wnode^1_2$};
            \node[main_node] (w_13) [right = 1.15 cm of w_12] {$\wnode^1_3$};
            \node[main_node] (p_11) [below right = 0.25 cm and 1.25 cm of s_1]  {$\pnode^1_1$};
            \node[node1] (t_1) [below right = 0.25 cm and 1.25 cm of w_13]  {$t^1$};
            
            \node (trans_node_1) [below left = 1 cm and 1.25 cm of s_1] {};
            \node (trans_node_2) [below left = 1 cm and 0.5 cm of s_1] {};
            \draw[ultra thick,->] (trans_node_1) to (trans_node_2);
            
            \path[edge]
                 (s_1) edge[bend left=20]  (w_11)
                 (w_11) edge[bend left=5] (w_12)
                 (w_12) edge[bend left=5] (w_13)
                 (w_13) edge[bend left=20] (t_1)
                 (s_1) edge[bend right=20]  (p_11)
                 (p_11) edge[bend right=15] (t_1);
        \end{scope}
        
        \begin{scope}[xshift=14.5cm, yshift=-3.25cm]
        
            \node[node2] (s_2) {$s^2$};
            \node[main_node] (w_21) [above right = 0.25 cm and 1.25 cm of s_2] { $\wnode^2_1$};
            \node[main_node] (w_22) [right = 1.15 cm of w_21] { $\wnode^2_2$};
            \node[main_node] (p_21) [below right = 0.25 cm and 1.25 cm of s_2]  {$\pnode^2_1$};
            \node[main_node] (p_22) [right = 1.15 cm of p_21]  {$\pnode^2_2$};
            \node[node2] (t_2) [below right = 0.25 cm and 1.25 cm of w_22]  {$t^2$};
            
            \node (info1) [below = 0.5 cm of p_22]  {(iii)};

            \path[edge]
                (s_2) edge[bend left=20]  (w_21)
                (w_21) edge[out=30,in=-80] (w_11)
                (w_22) edge[bend left=20] (t_2)
                (w_12) edge[out=-80,in=150] (w_22)
                (s_2) edge[bend right=20]  (p_21)
                (p_21) edge[out=80,in=-50] (w_12)
                (w_13) edge[out=-70,in=80] (p_22)
                (p_22) edge[bend right=15] (t_2);
                
            \path[highlighted edge]
                (s_2) to[bend right=20]  (p_21)
                (p_21) to[out=80,in=-50] (w_12)
                (w_12) to[bend left=5] (w_13)
                (w_13) to[out=-70,in=80] (p_22)
                (p_22) to[bend right=15] (t_2);


            \path[edge]
                (w_12) edge[line width = 2.5pt, bend left=5] (w_13);
        \end{scope}
    \end{tikzpicture}
    }
    \caption{Illustration of the re-routing of lightpaths in the {\PRWAreq} network $\exPRWAnetwork$ }
    \label{fig:nphard_path_constr}
\end{figure}

==> OnlineSupplement_subfiles/lemma_beta_models_equiv.tex <==
\begin{lemma}
\label{lem:beta_models_equiv} [?????]
The models in \eqref{eq:prioritization_optmodel0} and \eqref{eq:prioritization_optmodel1} yield the same optimal values; that is, $\LBprioOne = \LBprioExact$. 
\end{lemma}

\proof{Proof.}
The feasible region of the model in \eqref{eq:prioritization_optmodel0} contains that of \eqref{eq:prioritization_optmodel1}, and hence $\LBprioOne \geq \LBprioExact$.
Moreover, since the condition in \eqref{eq:prioritization_optmodel1} implies \eqref{eq:prioritization_optmodel0} by Proposition \ref{prop:beta_model_onediff}, we have that $\LBprioOne \leq \LBprioExact$, which establishes that they are equal. \Halmos

==> QUBO_subfiles/prop_penalty_tight_ex.tex <==
\begin{proposition}[Tight example for the penalty selection]
\label{prop:penalty_coef_tightLB} 
There exist {\PRWA} instances for which the sufficient condition for the penalty coefficient $\penaltyCoef$ given in \eqref{eq:penalty_coef_lb} is necessary as well.
%suggested in Proposition \ref{prop:penalty_coef} is necessary as well.

% |R| = 1, Wr = Pr, |Wr| = |Pr| = 1, w and p are not disjoint
% Only IP feasible: x = y = 0
% Necessary condition: rho >= max_{(x,y) binary s.t. g(x,y) >= 1} (f(x^*,y^*) - f(x,y)) / g(x,y)
% Unique maximizer: x = 1, y = 0
\end{proposition}
%
%

